Equivariant Light Field Convolution and Transformer

3D reconstruction and novel view rendering can greatly benefit from geometric priors when the input views are not sufficient in terms of coverage and inter-view baselines. Deep learning of geometric priors from 2D images often requires each image to be represented in a $2D$ canonical frame and the prior to be learned in a given or learned $3D$ canonical frame. In this paper, given only the relative poses of the cameras, we show how to learn priors from multiple views equivariant to coordinate frame transformations by proposing an $SE(3)$-equivariant convolution and transformer in the space of rays in 3D. This enables the creation of a light field that remains equivariant to the choice of coordinate frame. The light field as defined in our work, refers both to the radiance field and the feature field defined on the ray space. We model the ray space, the domain of the light field, as a homogeneous space of $SE(3)$ and introduce the $SE(3)$-equivariant convolution in ray space. Depending on the output domain of the convolution, we present convolution-based $SE(3)$-equivariant maps from ray space to ray space and to $\mathbb{R}^3$. Our mathematical framework allows us to go beyond convolution to $SE(3)$-equivariant attention in the ray space. We demonstrate how to tailor and adapt the equivariant convolution and transformer in the tasks of equivariant neural rendering and $3D$ reconstruction from multiple views. We demonstrate $SE(3)$-equivariance by obtaining robust results in roto-translated datasets without performing transformation augmentation.

==> comment_material.tex <==















==> table4.tex <==
\begin{table}
\scalebox{1.0}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
    Method &\multicolumn{3}{|c|}{I/I}&\multicolumn{4}{|c|}{I/SO(3)}\\
    \hline
    &PSNR$\uparrow$&SSIM$\uparrow$&LPIPS$\downarrow$&PSNR$\uparrow$&SSIM$\uparrow$&LPIPS$\downarrow$&Pixel Variance$\downarrow$\\ 
     \hline
    \multicolumn{8}{|c|}{Realistic Synthetic $360^{\circ}$ \cite{mildenhall2021nerf}}\\
    \hline %
    IBRNet\cite{wang2021ibrnet}&\textbf{26.91} & 0.928&\textbf{0.084}&26.77 &0.923 &0.091 & 66.58\\
    Ours&26.90 & \textbf{0.929}&0.086&\textbf{26.90}&\textbf{0.929} &\textbf{0.086}&\textbf{0.00}\\
      \hline
    \multicolumn{8}{|c|}{Real Forward-Facing \cite{mildenhall2019local}}\\
    \hline
    IBRNet\cite{wang2021ibrnet}& \textbf{25.13}&\textbf{0.817} &\textbf{0.205} &24.60 & 0.797&0.223 & 52.66\\
    Ours&24.93 &0.808 &0.212 &\textbf{24.93} &\textbf{0.808} &\textbf{0.212} &\textbf{0.00}\\
    \hline
    \multicolumn{8}{|c|}{Diffuse Synthetic $360^{\circ}$ \cite{sitzmann2019deepvoxels}}\\
    \hline
    IBRNet \cite{wang2021ibrnet} &\textbf{37.21} & \textbf{0.989}&\textbf{0.019} & 37.07& \textbf{0.988}& \textbf{0.019}&34.51 \\
    Ours& 37.11& 0.987& \textbf{0.019}&\textbf{37.11} & 0.987&\textbf{0.019} &\textbf{0.00}\\
\bottomrule
\end{tabular}
}
\caption{The results for the experiments of generalized rendering without per-scene tuning. The metrics in the cell are PSNR$\uparrow$, SSIM$\uparrow$ and Pixel Variance$\downarrow$. The evaluation of IBRNet\cite{wang2021ibrnet} is performed by testing the released model on both canonical and rotated test datasets.}
  \label{tab:rendering_table}
\end{table}


==> tutorial_blog.tex <==
\section{Part I}


\section{Part II}

\section{Part III}

\section{Part IV}
